PixArt-$\alpha$: Fast Training of Diffusion Transformer for Photorealistic Text-to-Image Synthesis

The most advanced text-to-image (T2I) models require significant training costs (e.g., millions of GPU hours), seriously hindering the fundamental innovation for the AIGC community while increasing CO2 emissions. This paper introduces PIXART-$\alpha$, a Transformer-based T2I diffusion model whose image generation quality is competitive with state-of-the-art image generators (e.g., Imagen, SDXL, and even Midjourney), reaching near-commercial application standards. Additionally, it supports high-resolution image synthesis up to 1024px resolution with low training cost, as shown in Figure 1 and 2. To achieve this goal, three core designs are proposed: (1) Training strategy decomposition: We devise three distinct training steps that separately optimize pixel dependency, text-image alignment, and image aesthetic quality; (2) Efficient T2I Transformer: We incorporate cross-attention modules into Diffusion Transformer (DiT) to inject text conditions and streamline the computation-intensive class-condition branch; (3) High-informative data: We emphasize the significance of concept density in text-image pairs and leverage a large Vision-Language model to auto-label dense pseudo-captions to assist text-image alignment learning. As a result, PIXART-$\alpha$'s training speed markedly surpasses existing large-scale T2I models, e.g., PIXART-$\alpha$ only takes 10.8% of Stable Diffusion v1.5's training time (675 vs. 6,250 A100 GPU days), saving nearly \$300,000 (\$26,000 vs. \$320,000) and reducing 90% CO2 emissions. Moreover, compared with a larger SOTA model, RAPHAEL, our training cost is merely 1%. Extensive experiments demonstrate that PIXART-$\alpha$ excels in image quality, artistry, and semantic control. We hope PIXART-$\alpha$ will provide new insights to the AIGC community and startups to accelerate building their own high-quality yet low-cost generative models from scratch.

==> figures_tex/pipeline_and_efficiency.tex <==
\begin{figure}[htbp]
    \begin{minipage}{.6\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/model.pdf}
    \caption{Model architecture of \model.}
    \label{fig:architecture}
        \label{fig:prob1_6_2}
    \end{minipage}
    \quad
    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/efficienct_data_usage.pdf}
        % \subcaption{1}
        \\
        \vspace{5pt}
        \includegraphics[width=\textwidth]{figures/efficienct_training_time.pdf}
        % \subcaption{1}
        \vspace{1pt}
    \caption{Comparison of the training time and the data usage mount with current popular diffusion models.}
    \label{fig:gflops_bubble}
    \end{minipage}
    \vspace{-8pt}
\end{figure}


==> figures_tex/traintime_data_compare.tex <==
\begin{figure}[ht]
\begin{center}
\footnotesize
\includegraphics[width=1\linewidth]{figures/traintime_data.pdf}
\caption{Comparison of the training time and the data usage mount with current popular diffusion models.}
\label{fig:traintime_data_compare}
\end{center} 
\end{figure}


==> tables/t2i_combench_new.tex <==
\begin{table}[ht]
\vspace{0pt}
\centering
    \caption{Benchmarking on T2I-CompBench.} 
    \vspace{0pt}
\label{benchmark:t2i_combench_all}
\resizebox{\linewidth}{!}{ 
\begin{tabular}
{lccccccccccc}
\toprule
\multicolumn{1}{c}
{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{2}{c}{\textbf{Color}}  &  \multicolumn{2}{c}{\textbf{Shape}} & \multicolumn{2}{c}{\textbf{Texture}}& \multicolumn{2}{c}{\textbf{Spatial}} & \textbf{Non-spatial} & \multicolumn{2}{c}{\textbf{Complex}}
\\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-10}\cmidrule(lr){11-12}

\multicolumn{1}{c}{}  & CLIP   & B-VQA    & CLIP   & B-VQA   & CLIP   & B-VQA   & CLIP   & UniDet    & CLIP      & CLIP   &3-in-1        \\
\midrule
Stable v1-4  & 0.3214 & 0.3765 & 0.3112 & 0.3576 & 0.3081 & 0.4156 & 0.3142 & 0.1246 & 0.3079 & 0.2876 & 0.3080  \\
\rowcolor{gray!15}
Stable v2 & 0.3335 & 0.5065 & 0.3203 & 0.4221 & 0.3185 & 0.4922 & 0.3206 & 0.1342 & 0.3127 & 0.3096 & 0.3386  \\
Dalle-2 & 0.3332 & 0.5750 & 0.3171 & 0.5464 &0.3188  &0.6374  & 0.3158 & 0.1283 & 0.3078 & 0.3043 & 0.3696(1)  \\
DeepFloyd & 0.3347 & 0.6430 &0.3209   &0.5845  & 0.3191 & 0.5947 & 0.3179 & 0.1786 & 0.3101 & 0.3109 &  0.4196(1) \\
SDXL & 0.3399 & 0.6674 & 0.3182 & 0.5642 & 0.3181 & 0.5709 & 0.3265 & 0.2072 & 0.3108 &0.3094  & 0.4137(1)  \\
SDXL-100seed & 0.3338 & 0.6064 & 0.3125 & 0.5174 & 0.3185 & 0.5565 & 0.3259 & 0.1992 & 0.3112 & 0.3085 & 0.4044(1)  \\
Composable v2 & 0.3178 & 0.4063 & 0.3092 & 0.3299 & 0.3092 & 0.3645 & 0.3001 & 0.0800 & 0.2980 & 0.3014 & 0.2898  \\
Structured v2 & 0.3319 & 0.4990 & 0.3178 & 0.4218 & 0.3167 & 0.4900 & 0.3201 & 0.1386 & 0.3111 & 0.3084 & 0.3355  \\
Attn-Exct v2 & 0.3374 & 0.6400 & 0.3189 & 0.4517 & 0.3171 & 0.5963 & 0.3213 & 0.1455 & 0.3109 & 0.2913 & 0.3401  \\
\rowcolor{gray!15}
GORS  & 0.3395 & 0.6603 & 0.2973 & 0.4785 & 0.3233 & 0.6287 & 0.3242 & 0.1815 & 0.3193 & 0.2973 & 0.3328  \\
\midrule
-mj256 & 0.3299 & 0.4070 & 0.3078 & 0.4714 & 0.3166 & 0.4902 & 0.3240 & 0.1884 & 0.3101 & 0.3068 & 0.4009(1)    \\
-mj512 & 0.3253 & 0.4714 & 0.3053 & 0.4887 & 0.3123 & 0.5217 & 0.3174 & 0.1837 & 0.3069 & 0.3038 & 0.4065(1)     \\
-sam80e & 0.3112 & 0.4682 & 0.2970 & 0.4087 & 0.3027 & 0.5699 & 0.3015 & 0.1173 & 0.2990 & 0.2931 & xx  \\
-sam120e & 0.3077 & 0.4530 & 0.2996 & 0.4266 & 0.3006 & 0.5611 & 0.2997 & 0.0995 & 0.2992 & 0.2925 & xx  \\
\midrule
-mj512-cfg2.0-bug-iddpm & 0.3185 & 0.4414 & 0.2959 & 0.4824 & 0.3009 & 0.5085 & 0.3080 & 0.1611 & 0.3009 & 0.2985 & 0.3872(1)    \\
-mj512-cfg2.5-bug-iddpm & 0.3223 & 0.4539 & 0.2999 & 0.4880 & 0.3055 & 0.5212 & 0.3116 & 0.1764 & 0.3040 & 0.3007 & 0.3946(1)    \\
-mj512-cfg3.0-bug-iddpm & 0.3246 & 0.4587 & 0.3041 & 0.4891 & 0.3090 & 0.5130 & 0.3153 & 0.1800 & 0.3058 & 0.3017 & 0.3989(1)    \\
\rowcolor{gray!15}
-mj512-cfg4.5-bug-iddpm & 0.3258 & 0.4812 & 0.3064 & \gain{0.5035} & 0.3123 & \gain{0.5193} & 0.3180 & \gain{0.2021} & 0.3078 & 0.3042 & \gain{0.4136(1)}  \\
-mj512-cfg4.5-bug-iddpm-seedcj & 0.3254 & 0.4458 & 0.3062 & 0.4970 & 0.3110 & 0.5306 &0.3062 & 0.2075 & 0.3085 & 0.3045 & 0.4084(1)  \\
-mj512-cfg4.5-bug-iddpm-seedjs & 0.3265 & 0.4474 & 0.3068 & 0.4856 & 0.3125 & 0.5345 & 0.3191 & 0.1916 &0.3072 & 0.3044 & 0.4147(1)  \\
-mj512-cfg4.5-bug-iddpm-seed43 & 0.3260 & 0.4586 & 0.3073 & 0.5030 & 0.3120 &0.5076 & 0.3207 & 0.2095 & 0.3086 & 0.3051 & 0.4115(1)  \\
-mj512-cfg5.0-bug-iddpm & 0.3263 & 0.4711 & 0.3081 & 0.4938 & 0.3130 & 0.5292 & 0.3189 & 0.2072 & 0.3081 & 0.3044 & 0.4131(1)  \\
-mj512-cfg5.5-bug-iddpm & 0.3260 & 0.4702 & 0.3073 & 0.4987 & 0.3143 & 0.5239 & 0.3198 & 0. 1925 & 0.3081 & 0.3046 & 0.4135(1)  \\
-mj512-cfg6.0-bug-iddp & 0.3264 &0.4682 & 0.3075 & 0.5069 & 0.3140 & 0.5299 & 0.3197 & 0.2054 & 0.3083 & 0.3054 & 0.4129(1)  \\
\rowcolor{gray!15}
-mj512-cfg7.0-bug-iddp & 0.3265 & 0.4631 & 0.3082 & 0.5152 & 0.3142 & 0.5348 & 0.3195 & 0.2192 & 0.3089 & 0.3053 & 0.4168(1)  \\
\midrule
-mj512-cfg4.5-bug-diipm-woft\_e1 & 0.3276 & 0.4510 & 0.3088 & 0.4723 & 0.3167 & 0.5488 & 0.3227 & 0.2126 & 0.3095 & 0.3062 & 0.3705(1)  \\
\midrule
-mj1024-cfg4.5-bug-iddpm & 0.3289 & 0.4722 & 0.3071 & 0.4622 & 0.3164 & 0.5428 & 0.3219 & 0.2291 & 0.3071 & 0.3052 & 0.3963(1)  \\
\midrule
-mj1024-cfg4.5-bug-dpms & 0.3322 & 0.4638 & 0.3085 & 0.4789 &0.3149 & 0.5349 & 0.3213 & 0.2182 & 0.3065 & 0.3065 & 0.4115(1)  \\
\midrule
-mj512-cfg2.0-fix-iddpm & 0.3185 & 0.4290 & 0.2976 & 0.4506 & 0.2994 & 0.4279 & 0.3098 & 0.1270 & 0.3010 & 0.2984 & 0.3853(1)    \\
-mj512-cfg2.5-fix-iddpm & 0.3214 & 0.4303 & 0.3003 & 0.4438 & 0.3050 & 0.4878 & 0.3140 & 0.1527 & 0.3037 & 0.3010 & 0.3928(1)    \\
-mj512-cfg3.0-fix-iddpm & 0.3217 & 0.4328 & 0.3012 & 0.4476 & 0.3072 & 0.4846 & 0.3178 & 0.1638 & 0.3049 & 0.3029 & 0.4008(1)    \\
\midrule
-mj512-cfg2.0-fix-dpms & 0.3211 & 0.4217 & 0.2974 & 0.4449 & 0.2993 & 0.4684 & 0.3112 & 0.1234 & 0.2991 & 0.3010 & 0.3888(11)  \\
-mj512-cfg3.0-fix-dpms & 0.3269 & 0.4365 & 0.3016 & 0.4311 & 0.3043 & 0.4682 & 0.3161 & 0.1655 & 0.3055 & 0.3049 & 0.3965(11)  \\
-mj512-cfg4.0-fix-dpms & 0.3287 & 0.4208 & 0.3041 & 0.4459 & 0.3077 & 0.4888 & 0.3194 & 0.1667 & 0.3064 & 0.3060 & 0.3975(11)  \\
\midrule
-mj512-cfg4.0-bug-dpms  & 0.3301 & 0.4485 & 0.3052 & 0.4723 & 0.3098 & 0.5187 & 0.3171 & 0.2009 & 0.3073 & 0.3070 & 0.4090(1)  \\
\midrule
-iddpm-single-e11 & 0.3270 & 0.4652 & 0.3064 & 0.4560 & 0.3125 & 0.4560 & 0.3202 & 0.2166 & 0.3071 & 0.3046 & 0.4059(1)  \\
\midrule
ft-2e-cfg4.5-512-iddpm &  0.3408 & 0.5711& 0.3157 &  0.4774 & 0.3225 & 0.5956 & 0.3261 & 0.1883 &  0.3137 & 0.3080 &  0.4163(1)  \\
ft-16e-cfg4.5-512-iddpm & 0.3395 & 0.6286 & 0.3157 & 0.5182 & 0.3276 & 0.6595 & 0.3274 & 0.1975 & 0.3143 & 0.3099 & 0.4193(1)  \\
ft-23e-cfg4.5-512-iddpm & 0.3402 & 0.6357 & 0.3191 & 0.5358 & 0.3270 & 0.6788 & 0.3274 &0.2113 & 0.3157&  0.3094  & 0.4176(1)  \\
ft-33e-cfg4.5-512-iddpm & 0.3392 & 0.6402 & 0.3156 &  0.4943 & 0.3269 &  0.6531 & 0.3293 & 0.2202 & 0.3156 & 0.3110 &  0.4097(1)  \\
ft-51e-cfg4.5-512-iddpm  & 0.3406 & 0.6467 & 0.3181 & 0.5229 & 0.3270 &  0.6765 & 0.3291 &  0.2180 &  0.3164  & 0.3107 & 0.4246(1)  \\
ft-59e-cfg4.5-512-iddpm & 0.3398 & 0.6457 & 0.3158 & 0.5480 & 0.3278 & 0.6851 & 0.3286 & 0.2259 & 0.3163 & 0.3089 &0.4135(1)  \\
\rowcolor{gray!15}
ft-85e-cfg4.5-512-iddpm & 0.3410 & 0.6979 & 0.3154 & 0.5221 & 0.3283 & 0.6749 & 0.3319 & 0.2216 & 0.3175 & 0.3099 &  0.4150(1)  \\
ft-90e-cfg4.5-512-iddpm & 0.3400 & 0.6738 & 0.3176 & 0.5351 & 0.3276 & 0.6818 & 0.3288 & 0.2187 & 0.3172 & 0.3104 & 0.4183(1)  \\
ft-95e-cfg4.5-512-iddpm & 0.3405 &0.6776 & 0.3177 & 0.5381 &0.3277 & 0.6705 & 0.3304 & 0.2194 & 0.3165 & 0.3100 & 0.4150(1)  \\
ft-100e-cfg4.5-512-iddpm & 0.3407 & 0.6677 & 0.3185 & 0.5268 & 0.3260 & 0.6705 & 0.3310 & 0.2362 & 0.3171 & 0.3096 & 0.4130(1)  \\
\midrule
85e-512-cfg2.0 (same?) & 0.3396 & 0.6648 & 0.3157 & 0.5207 & 0.3214 & 0.6524 & 0.3295 & 0.1775 & 0.3158 & 0.3077 & 0.4096(1)  \\
85e-512-cfg2.5 & 0.3396 & 0.6648 & 0.3157 & 0.5207 & 0.3214 & 0.6524 & 0.3295 & 0.1775 & 0.3158 & 0.3077 & 0.4096(1)  \\
85e-512-cfg3.0 & 0.3414 & 0.6811 & 0.3175 & 0.5260 & 0.3269 & 0.6609 & 0.3305 & 0.1865 & 0.3160 & 0.3088 & 0.4112(1)  \\
85e-512-cfg4.0 & 0.3429 & 0.6911 & 0.3186 & 0.5418 & 0.3286 & 0.6800 & 0.3313 & 0.1919 & 0.3165 & 0.3110 & 0.4082(1)  \\
85e-512-cfg4.5 & 0.3411 & 0.6731 & 0.3172 & 0.5430 & 0.3293 & 0.6850 & 0.3308 & 0.1861 & 0.3187 & 0.3095 & 0.4059(1)  \\
85e-512-cfg5.0 & 0.3417 & 0.6832 & 0.3198 & 0.5441 & 0.3280 & 0.6939 & 0.3305 & 0.2130 & 0.3184 & 0.3118 & 0.4163(1)  \\
85e-512-cfg5.5 & 0.3428 & 0.6886 & 0.3194 & 0.5582 & 0.3286 & 0.7044 & 0.3325 & 0.2082 & 0.3179 & 0.3126 &  0.4117(1)  \\
85e-512-cfg6.0 & 0.3438 & 0.7019 & 0.3189 & 0.5530 & 0.3301 & 0.7021 & 0.3324 & 0.2111 & 0.3186 & 0.3108 & 0.4128(1)  \\
85e-512-cfg7.0 & 0.3431 & 0.6913 & 0.3182 & 0.5588 & 0.3279 & 0.6971 & 0.3320 & 0.1933 & 0.3188 & 0.3122 & 0.4115(1)  \\
\midrule
85e-512-cfg2.5-sas & 0.3392 & 0.6482 & 0.3183 & 0.5226 & 0.3252 & 0.6539 & 0.3285 & 0.2105 & 0.3158 & 0.3087 &  0.4133(1)  \\
85e-512-cfg3.0-sas & 0.3396 & 0.6445 & 0.3178 & 0.5173 & 0.3241 & 0.6727 & 0.3299 & 0.2121 & 0.3164 & 0.3099 &  0.4149(1)  \\
85e-512-cfg4.0-sas & 0.3407 & 0.6568 & 0.3155 & 0.5279 & 0.3281 & 0.6749 & 0.3303 & 0.1880 & 0.3184 & 0.3107 & 0.4128(1)  \\
85e-512-cfg5.0-sas & 0.3420 & 0.6734 & 0.3181 & 0.5227 & 0.3264 & 0.6573 & 0.3302 & 0.2427 & 0.3174 & 0.3104 & 0.4057(1)  \\
85e-512-cfg6.0-sas & 0.3421 & 0.6321 & 0.3178 & 0.5316 & 0.3268 & 0.6701 & 0.3302 & 0.2118 & 0.3173 & 0.3112 & 0.4210(1)  \\
85e-512-cfg7.0-sas & 0.3413 & 0.6815 & 0.3191 & 0.5597 & 0.3277 & 0.6886 & 0.3294    & 0.1795 & 0.3169 & 0.3107 &  0.4119(1)  \\
\midrule
expname & xx & xx & xx & xx & xx & xx & xx & xx & xx & xx & xx  \\
\bottomrule
\end{tabular}
}
\vspace{0pt}
\end{table}
